New Feedback Control and Adaptive Evolve-Filter-Relax Regularization for the Navier-Stokes Equations in the Convection-Dominated Regime

We propose, analyze, and investigate numerically a novel feedback control strategy for high Reynolds number flows. For both the continuous and the discrete (finite element) settings, we prove that the new strategy yields accurate results for high Reynolds numbers that were not covered by current results. We also show that the new feedback control yields more accurate results than the current control approaches in marginally-resolved numerical simulations of a two-dimensional flow past a circular cylinder at Reynolds numbers $Re=1000$. We note, however, that for realistic control parameters, the stabilizing effect of the new feedback control strategy is not sufficient in the convection-dominated regime. Our second contribution is the development of an adaptive evolve-filter-relax (aEFR) regularization that stabilizes marginally-resolved simulations in the convection-dominated regime and increases the accuracy of the new feedback control in realistic parameter settings. For the finite element setting, we prove that the novel feedback control equipped with the new aEFR method yields accurate results for high Reynolds numbers. Furthermore, our numerical investigation shows that the new strategy yields accurate results for reduced order models that dramatically decrease the size of the feedback control problem.

==> sections/Numerical_uncontrolled.tex <==
\section{EFR and EFR-EFR for NSE: a parametric study}
\label{app:EFRapp}
This section %focuses on the need for the EFR algorithm for Navier-Stokes both at the FOM and at the ROM level.
{is a numerical investigation of the increased stability and accuracy of the EFR strategy for FOM and ROM marginally-resolved simulations.}
We perform two {numerical} experiments.
\begin{itemize}
    \item [$\circ$] \emph{Experiment A1}. A numerical comparison between noEFR and EFR at the FOM level. %This 
    {In particular, this} experiment analyzes the performance of the EFR algorithm %changing $\delta$, giving some guidelines for the more convenient value to use in 
    {for different $\delta$ values, providing guidelines for} 
    the numerical setting of section \ref{exp1:fafb}. 
    \item [$\circ$] \emph{Experiment A2}. A numerical comparison between noEFR and EFR at the ROM level %once performed EFR to obtain the 
    {for} POD basis functions {obtained by using the EFR regularization}.
\end{itemize}

\subsection{{noEFR vs. EFR Numerical Comparison (Experiment A1)}}
\label{sec:exampleFOM}
In this section, we perform a numerical investigation of the role played by the EFR strategy in %under-resolved \ms{
marginally-resolved FOM simulations.
To this end, we compare the following two approaches:
(i) noEFR, which is a standard numerical discretization of the NSE without the EFR regularization; and 
(ii) EFR, which is a %standard 
numerical discretization of the NSE with %an 
the EFR regularization.
{We now focus on the uncontrolled framework, which is extended to the feedback control setting in section \ref{sec:problem}. In this section, we solve problem \eqref{eq:NSE}. The domain and the boundary conditions are %the ones considered 
{those used} in {section} \ref{sec:examplecontrolFOM}. The initial condition is $u_0 = (0,0)$, %we simulate in 
the time interval {is} $(0,4)$, and {the time step is} $\Delta t = 4\cdot 10^{-4}$. We %build a new 
{use a} test case that highlights the %criticalities 
{drawbacks} of the noEFR procedure in marginally-resolved regimes.} 
We remark that, differently from \cite{Strazzullo20223148}, where %they 
%they work with 
{the range of the Reynolds number is} $0 \leq Re \leq 100$, we %are working 
{work} with a %significantly larger 
Reynolds number that is { one order of magnitude higher}: $Re = 1000$. 
The first questions we address are: (i) How do the mesh parameters affect the stability of the noEFR solutions? %in terms of accuracy 
and (ii) Are the simulations {accurate?} %feasible?
The numerical investigation %is pursued over 
{employs} four meshes: M1, M2, M3, and M4. M1 is the mesh depicted in Figure \ref{fig:mesh}. We recall {that} the mesh parameters {are} %:
 $h_{min} = 4.46 \cdot 10^{-3}$ and $h_{max} = 4.02 \cdot 10^{-2}$. To solve the system, we employ {the} Taylor-Hood $\mathbb P^2 - \mathbb P^1$ %FE 
 {finite element} discretization for velocity and pressure, respectively, with $N_h \doteq N_h^{u} + N_h^p = 14053$ degrees of freedom. M2 is a finer mesh with $h_{min} = 4.45 \cdot 10^{-3}$ and $h_{max} = 1.67 \cdot 10^{-2}$, and $N_h = 68117$. We %analyzed also 
 {also analyze} the performance of M3, a finer mesh with respect to M2 and M1, with $h_{min} = 4.45 \cdot 10^{-3}$ and $h_{max} = 1.49 \cdot 10^{-2}$, and $N_h = 93076$. The finest mesh is %M3 
 {M4}, with $h_{min} = 4.44 \cdot 10^{-3}$ and $h_{max} = 1.13 \cdot 10^{-2}$, and $N_h = 113436$. Table \ref{tab:meshval} summarizes the parameters of the %three 
 {four} meshes. 
 \begin{table}[H]
\caption{Experiment A1. Comparison of the M1, M2, M3, and M4 with respect to $h_{min}$, $h_{max}$, and number of %dofs.
{degrees of freedom}.}
\label{tab:meshval} \centering
\begin{tabular}{|c|c|c|c|}
\hline
mesh & $h_{min}$            & $h_{max}$            &  $N_h$     \\ \hline
M1   & $4.46\cdot 10^{-3}$  & $4.02 \cdot 10^{-2}$ & $14053$  \\ \hline
M2   & $4.45\cdot 10^{-3}$  & $1.67\cdot 10^{-2}$  & $68117$  \\ \hline
M3   & $4.45\cdot 10^{-3}$  & $1.49\cdot 10^{-2}$  & $93076$  \\ \hline
M4  & $4.44 \cdot 10^{-3}$ & $1.13\cdot 10^{-2}$  & $113436$ \\ \hline
\end{tabular}
\end{table}

\begin{figure}[H]
  \centering
  \includegraphics[width=0.48\textwidth]{img/uncontrolled/M1noEFR.png}  
  \includegraphics[width=0.48\textwidth]{img/uncontrolled/M2noEFR.png} \\
  \includegraphics[width=0.49\textwidth]{img/uncontrolled/M3noEFR.png} \includegraphics[width=0.49\textwidth]{img/uncontrolled/M4noEFR.png} 
  \caption{Experiment A1. noEFR vs EFR. noEFR velocity profile for $t=4$ and M1 (top left plot), M2 (top right plot), M3 (bottom left plot), and M4 (bottom right plot).}
  \label{fig:nocontrolvscontrolmesh}
\end{figure}

\begin{figure}[H]
  \centering
  \includegraphics[width=0.47\textwidth]{img/uncontrolled/norm.pdf}
  \includegraphics[width=0.46\textwidth]{img/uncontrolled/segdai.png}\\
   
  \caption{Experiment A1. noEFR vs EFR. $L^2$ velocity norm and velocity magnitude over $\Gamma_N$ for M1 (dashed green line), M2 (solid magenta line), and M3 (dashed-dotted orange line), left and right plot, respectively.
  }
  \label{fig:norm}
  \end{figure}  

 With M1, as stated in \cite{Strazzullo20223148}, we %are working 
 {work} in a marginally-resolved regime. For high {Reynolds number} values, %of $Re$, 
 the simulation does not capture the features of the flow, presenting numerical oscillations, %. This is evident 
 {as illustrated} in the top left plot of Figure \ref{fig:nocontrolvscontrolmesh}. The numerical oscillations are alleviated {by decreasing} %diminishing 
 the value of $h_{max}$. %While for 
 {For} M2, we can observe some oscillations just {behind} %passed 
 the cylinder and at the end of the channel. These %latter 
 oscillations remain even {by} decreasing the value of $h_{max}$, as done for M3 and M4. However, these meshes are capable of smoothly representing the vortex shedding. 
 Moreover, %for 
 the $L^2$-norm plot in Figure \ref{fig:norm} shows that {the numerical results on} M3 and M4 are comparable, and their norms %reaches a convergent behaviour, 
 {converge}, %which is not recovered from 
 {whereas the numerical results on} M1 and M2 {are far apart}. The right plot of Figure \ref{fig:norm} shows the magnitude of the velocity field for M3 and M4 over the %homogeneous Neumann 
 {``free flow"} boundary $\Gamma_N$. As expected, M4 presents smaller magnitude values for the oscillations at the end of the channel with respect to M3. 


 \begin{figure}[H]
        \centering \hspace{-5mm}\includegraphics[scale=0.25]{img/uncontrolled/M4noEFR.png}
        \centering  \hspace{-5mm}\includegraphics[scale=0.25]{img/uncontrolled/EFR375.png}\\
        \centering \includegraphics[scale=0.25]{img/uncontrolled/EFR4.png}
        \centering \includegraphics[scale=0.25]{img/uncontrolled/EFR45.png}\\
        \centering \includegraphics[scale=0.25]{img/uncontrolled/EFR5.png}
        \centering \includegraphics[scale=0.25]{img/uncontrolled/EFR55.png}
        

\caption{{Experiment A1. noEFR vs EFR. {noEFR over} M4 (top left plot) vs EFR over M1 for several values of $C_{\delta}$ and $t=4$.}
\label{fig:compEFR}
}\end{figure}

\begin{figure}[H]
  \centering
  \includegraphics[width=0.468\textwidth]{img/uncontrolled/efrnorm.pdf}
  \includegraphics[width=0.49\textwidth]{img/uncontrolled/efrerr.pdf}
  \caption{{Experiment A1. noEFR vs EFR. (left plot) $L^2$ velocity norm for EFR strategy with $C_{\delta} \in \{ \sqrt{7.5}, \sqrt{8}, \sqrt{9}, \sqrt{10}, \sqrt{11}\}$. The results are compared with the noEFR $L^2$ velocity norm for M4. (Right plot) Relative errors between EFR strategy and M4 with $C_{\delta} \in \{ \sqrt{7.5}, \sqrt{8}, \sqrt{9}, \sqrt{10}, \sqrt{11}\}$.}}
  \label{fig:normefr}
  \end{figure} 
We conclude that M4 is %a valuable 
{an appropriate} choice to accurately represent the flow past %Cylinder 
{a cylinder} for $Re=1000$. %and we will use it as a term of comparison for 
{Thus, we will use %it 
{M4} as a benchmark to answer} 
the following question: %\\ 
Is it possible to %exploit 
{use} M1 and %use 
EFR to %reach more accurate results, say one of the finest mesh M4? 
{obtain results that are as accurate as those obtained on the finest mesh, M4?}
% In other words: is EFR useful? \\

At the FOM level, %if one is 
in the marginally-resolved regime, the EFR algorithm %was necessary to deal with this value of $Re$. 
{is needed to stabilize the simulation.}
Indeed, when no EFR algorithm %was 
{is} employed, nonphysical numerical oscillations can be observed for %velocity 
the velocity field, as already shown in the top left plot of Figure \ref{fig:nocontrolvscontrolmesh}.
In contrast, the EFR algorithm is able to alleviate the oscillations arising %from 
{in} convection-dominated problems and %allows us to reach a physical simulation. 
{yields more accurate results.}
Following %the tips of other work in 
{the suggestions found in, e.g., }
%literature, see e.g.\ 
\cite{bertagna2016deconvolution,Strazzullo20223148}, we use $\chi = 5\cdot \Delta t$. However, we try different values of the differential filter radius, {$\delta$}. 
  \begin{figure}[H]
  \centering
  \includegraphics[width=0.49\textwidth]{img/uncontrolled/last_comp11_norms.pdf}
  \includegraphics[width=0.485\textwidth]{img/uncontrolled/err11.pdf}
  \caption{{Experiment A1. noEFR vs EFR. (left plot) $L^2$ velocity norm for noEFR and EFR %strategy 
  {strategies} with $C_{\delta} = \sqrt{11}$. The results are compared with the noEFR $L^2$ velocity norm for M4 (solid starred-red line). (Right plot) Relative errors of noEFR and EFR $C_{\delta} = \sqrt{11}$ strategies with respect to the simulation on M4.}
  }
  \label{fig:compEFRnoEFR}
  \end{figure} 
 
We first define a reference value, %say $\delta^*$ with 
$\delta^* = 4.46\cdot 10^{-3}$, i.e., the $h_{min}$ value of M1 (see \cite{Strazzullo20223148}). %The idea is of increasing 
{Our goal is to increase} the action of the differential filter over the domain. %To do so, we increased 
{To this end, we increase} the reference value by a multiplicative constant, i.e., {we consider} $\delta = C_{\delta} \delta^*$. We %tried 
{try} several values for $C_{\delta}$ and, for the sake of brevity, we show {only} the results for $C_{\delta} \in \{ \sqrt{7.5}, \sqrt{8}, \sqrt{9}, \sqrt{10}, \sqrt{11}\}$. %\\

All the values are able to recover, with a certain degree of accuracy depending on $\delta$, the vortex shedding of the M4 simulation, as shown in Figure \ref{fig:compEFR}. %In terms of 
{With respect to the} $L^2$-norm of the velocity (left plot of Figure \ref{fig:normefr}), for all the choices of $C_{\delta}$, we obtain comparable results {on the entire time interval.} %and they 
{These results} are very similar to the reference value for $t \in (0,1)$, %. For $t>1$, the difference is larger. 
{but are significantly different from the reference value for $t \in (1,4)$.}
%To understand what was the better parameter to choose as $\delta$, 
{To study the optimal $\delta$ value,} 
we also investigate the relative error between the EFR strategy and the simulation obtained %by means of 
{on the finest mesh,} M4 (right plot of Figure \ref{fig:normefr}). %From the plot, it is clear that for $C_{\delta} > {\sqrt{7.5}}$, the EFR strategy presents similar results, however, for $t>2$, the minimum of the error is obtained for $t \sim 3.25$ by $C_{\delta} = \sqrt{11}$. We also observe that for $t \in (1,2)$ the smallest value of $C_{\delta}$ performs better than the others. However, for $t \in (2,3.5)$ the relative error drastically increases. For this reason, we believe that in this context $C_{\delta} = \sqrt{11}$ is the best parameter we can choose between the ones analyzed.\\
{This plot shows that $C_{\delta} = \sqrt{7.5}$ yields the most accurate results on {the time intervals} $(1,2)$ and $(3.75,4)$, and $C_{\delta} = \sqrt{11}$ yields the most accurate results on {the time intervals} $(2.5,3.75)$.
On the average, $C_{\delta} = \sqrt{11}$ seems to yield the most accurate results.}

The performance of the EFR strategy with respect to noEFR in terms of $L^2$ velocity norm and relative error %are depicted 
{is displayed} in Figure \ref{fig:compEFRnoEFR}. %From the plots is evident 
{These plots show that the EFR regularization is more accurate,} %that applying the EFR regularization is beneficial in terms of accuracy, 
with an error that is around $65\%$ smaller for $t>1.25$ (right plot) and a better representation of the $L^2$ velocity norm (left plot). %\\

%{Do we really need the next two sentences?  I think we could take them off.  Or move them to conclusions?}
%We stress that our goal was to show that EFR is a valuable strategy to deal with convection-dominated flows in marginally-resolved regimes. Performing a sensitivity analysis for $\delta$ and $\chi$ is beyond the scope of this contribution.

\begin{comment}

\begin{figure}[H]
  \centering
  \includegraphics[width=0.49\textwidth]{img/uncontrolled/segmentEFR1.pdf}
  \includegraphics[width=0.49\textwidth]{img/uncontrolled/segmentEFR2.pdf}
  \caption{noEFR vs EFR. EFR velocity magnitude on $\sigma$ with $C_{\delta} \in \{ \sqrt{7.5}, \sqrt{8}, \sqrt{9}\}$ in the left plot and $C_{\delta \in \{}\sqrt{10}, \sqrt{11}\}$ in the right plot. The results are compared with the noEFR velocity magnitude for M4.}
  \label{fig:segment1efr}
  \end{figure}


\begin{figure}[H]
  \centering
  \includegraphics[width=0.49\textwidth]{img/uncontrolled/gammaefr3.pdf}
  \includegraphics[width=0.49\textwidth]{img/uncontrolled/gammaefr1.pdf}
  \caption{noEFR vs EFR. EFR velocity magnitude on $\Gamma_N$ with $C_{\delta} \in \{ \sqrt{7.5}, \sqrt{8}, \sqrt{9}\}$ in the left plot and $C_{\delta \in \{}\sqrt{10}, \sqrt{11}\}$ in the right plot. The results are compared with the noEFR velocity magnitude for M4.}
  \label{fig:segment2efr}
  \end{figure}
 \todo{add some plot with noEFR M1 and $C_{\delta}=\sqrt{11}$ and comment} 
\begin{comment}

The space domain is $\Omega \doteq \{[0, 2.2] mes [0, 0.41]\} \setminus \{(x, y)\in \mathbb R^2 \text{ such that } (x - 0.2)^2 + (y - 0.2)^2 - 0.05^2 = 0 \}$, represented in Figure \ref{fig:domain}. 
The Dirichlet boundary condition is 
\begin{equation}
\label{eq:inlet}
u_D = 
\begin{cases}
0 & \text{ on } \Gamma_W, \\
u_{\text{in}} = \displaystyle \left  ( \frac{6}{0.41^2}y(0.41 - y), 0 \right) & \text{ on } \Gamma_{\text{in}}
\end{cases}
\end{equation}
where $\Gamma_W$ %is 
are the bottom ($\Gamma_B$) and the top ($\Gamma_T$) walls of the channel together with the walls of the cylinder ($\Gamma_C$) (solid teal boundary in Figure \ref{fig:domain}). The inlet condition $u_{\text{in}}$ is applied to $\Gamma_{\text{in}} = \{0\} mes [0, 0.41]$, (magenta dashed line in Figure \ref{fig:domain}). The prescribed inlet condition is given by equation \eqref{eq:inlet}.
Moreover, $\Gamma_N$ (black dotted boundary in Figure \ref{fig:domain}) features homogeneous Neumann conditions.

    
At the FOM level, the EFR algorithm was necessary to deal with this value of $Re$. Indeed, when no EFR algortihm was employed, nonphysical numerical oscillations can be observed in both for velocity and pressure fields in Figure \ref{fig:comp_uncontrol_v}
\ms{Do you thing the filtering is enough? Do I have to increase $\delta$?}
{In contrast, the} EFR algorithm is able to alleviate the oscillations arising from convection-dominated problems and allows to reach a physical simulation. The differential filter radius is $\delta = 1.22\cdot 10^{-2}$ and $\chi = 5\cdot \Delta t$. The relaxation parameter is the one used in \cite{Strazzullo20223148}, the filter radius is chosen in the following way. \ms{I am trying the parameter that suited for the unsteady BCs problem}


%We took the reference value of the filtered radius as in \cite{Strazzullo20223148}, say $ \hat{\delta}=(\sqrt{2})\delta^* $ with $\delta^* = 4.46\cdot 10^{-3}$ and %we choose 
%chose $\delta$ as the minimum value in the set \todo{change the values, they are not correct, see code on the EFR-EFR folder} 
%$\{\sqrt{2}\delta^*,\sqrt{2.25}\delta^*, \sqrt{2.5}\delta^*,\sqrt{2.75}\delta^*, \sqrt{3}\delta^*, \sqrt{3.25}\delta^*, \sqrt{3.5}\delta^*, \sqrt{3.75}\delta^*, \sqrt{4}\delta^*\}$ that guarantees the convergence of the Newton's solver. 

 

 

 Specifically, $\delta =\sqrt{7.5}\delta^*= 1.22\cdot 10^{-2}$. The idea of increasing the action of the differential filter over the domain. To do so, we increased the multiplicative value in front of $\delta^*$ with a trial-and-error approach. This is shown in Figures \ref{fig:Netwon_v} and \ref{fig:Netwon_p}: they represent velocity and pressure fields for $t = 0.4, 1.2, 4$ for standard NS with noEFR (left plots) and EFR (right plots). 
 \begin{figure}
        \centering \includegraphics[scale=0.25]{img/uncontrolled/nocontrol04.png}
        \centering  \includegraphics[scale=0.25]{img/uncontrolled/EFR_04.png}\\
        \centering \includegraphics[scale=0.25]{img/uncontrolled/nocontrol12.png}
        \centering \includegraphics[scale=0.25]{img/uncontrolled/EFR_12.png}\\
        \centering \includegraphics[scale=0.25]{img/uncontrolled/nocontrol4.png}
        \centering \includegraphics[scale=0.25]{img/uncontrolled/EFR_4.png}
        

\caption{\scriptsize{Representative FOM solutions for velocity: noEFR (left plots) and EFR (right plots). From top to bottom: $t=0.4$, $t=1.2$, $t=4$.}
\label{fig:comp_uncontrol_v}
}\end{figure}

\begin{figure}
        \centering \includegraphics[scale=0.25]{img/uncontrolled/FE1.png}
        \centering  \includegraphics[scale=0.25]{img/uncontrolled/EFR386.png}\\
        \centering \includegraphics[scale=0.25]{img/uncontrolled/FE2.png}
        \centering \includegraphics[scale=0.25]{img/uncontrolled/EFR39.png}\\
        \centering \includegraphics[scale=0.25]{img/uncontrolled/FE3.png}
        \centering \includegraphics[scale=0.25]{img/uncontrolled/EFR394.png}
        

\caption{\scriptsize{Representative FOM solutions for velocity: no-EFR (left plots) and EFR (right plots). From top to bottom: $t=3.86$, $t=3.9$, $t=3.94$.}
\label{fig:Netwon_v}
}\end{figure}


\begin{figure}[H]
        \centering \includegraphics[scale=0.25]{img/uncontrolled/FE1_p.png}
        \centering 
        \includegraphics[scale=0.25]{img/uncontrolled/pEFR386.png}\\
        \centering \includegraphics[scale=0.25]{img/uncontrolled/FE2_p.png}
        \centering \includegraphics[scale=0.25]{img/uncontrolled/pEFR39.png}\\
        \centering \includegraphics[scale=0.25]{img/uncontrolled/FE3_p.png}
        \centering \includegraphics[scale=0.25]{img/uncontrolled/pEFR394.png}
        

\caption{\scriptsize{Representative FOM solutions for pressure: no-EFR (left plots) and EFR (right plots). From top to bottom: $t=3.86$, $t=3.9$, $t=3.94$.}
\label{fig:Netwon_p}
}\end{figure}





\begin{figure}
  \centering
  \includegraphics[width=0.49\textwidth]{img/uncontrolled/energy_v.pdf}
  \includegraphics[width=0.49\textwidth]{img/uncontrolled/energy_p.pdf}\\
   
  \caption{FE (teal dashed line) and EFR (magenta solid line) velocity and pressure $L^2-$norm in $(0, 3.94)$ for $\nu=10^{-4}, \delta=1.22\cdot 10^{-2}, \chi = 5\cdot \Delta t$, left and right plot, respectively}
  \label{fig:blow-up}
  \end{figure}
\subsection{{EFR-noEFR vs. EFR-EFR Numerical Comparison}}
In this section, we perform a numerical investigation of the role played by the EFR strategy in under-resolved ROM simulations.
To this end, we compare the following two approaches:
(i) EFR-noEFR, which is the standard G-ROM without an EFR regularization; and 
(ii) EFR-EFR, which is the standard G-ROM with an EFR regularization.
The FOM setting is the EFR presented in section \ref{sec:uncontroled_example}. \\ We recall the parameters used. The triangular mesh parameters are
 $h_{min} = 4.46 \cdot 10^{-3}$ and $h_{max} = 4.02 \cdot 10^{-2}$ and by means of a Taylor-Hood $\mathbb P^2 - \mathbb P^1$ FE discretization we have $N_h \doteq N_h^{u} + N_h^p = 14053$ degrees of freedom. Moreover, $\nu = 10^{-4}$ ($Re = 1000$), $T=8 - \Delta t \sim 8$, for $\Delta t = 4\cdot 10^{-4}$, $\delta = 1.22\cdot 10^{-2}$ and $\chi = 5\cdot \Delta t$.\\
 For the EFR-EFR algorithm, we followed the consistency strategy proposed in \cite{Strazzullo20223148} and these parameters are used both at the FOM and at the ROM level. We show representative solutions in Figure \ref{fig:comp_uncontrolled}. \todo{add plots}The left plot are the EFR, EFR-noEFR and EFR-EFR velocity profiles for $t=4$, from top to bottom. Analogously, the pressure fields for the different strategies are represented in the right column of Figure \ref{fig:comp_uncontrolled}. 
 \todo{change the part below according to the new results}
 
\end{comment}

\subsection{{EFR-noEFR vs. EFR-EFR Numerical Comparison (Experiment A2)}}
\label{sec:compnocontrol}

In this section, we perform a numerical investigation of the role played by the EFR strategy in under-resolved ROM simulations.
To this end, we compare the following two approaches:
(i) EFR-noEFR, which is the standard G-ROM without an EFR regularization; and 
(ii) EFR-EFR, which is the %standard 
G-ROM with an EFR regularization.


 \begin{figure}[H]
  \centering
  \includegraphics[width=0.49\textwidth]{img/uncontrolled/EFR55bis.png}  \\
  \includegraphics[width=0.49\textwidth]{img/uncontrolled/EFR20.png}\includegraphics[width=0.49\textwidth]{img/uncontrolled/EFREFR20.png}
  \caption{Experiment A2. EFR-noEFR vs EFR-EFR. Top plot: EFR velocity profile for $t=4$. Bottom plot: EFR-noEFR {(left)} and EFR-EFR {(right)}. %left and right plots, respectively.
  }
  \label{fig:EFRvsnoEFRrom}
\end{figure}

  \begin{table}[H]
\caption{Experiment A2. %Energy 
{Information} retained %from 
{by} the POD basis functions for velocity and pressure.}
\label{tab:A2energy} \centering
\begin{tabular}{|c|c|c|}
\hline
$r_u = r_p$& Velocity %Energy 
{Information}           & Pressure %Energy  
{Information}             \\ \hline
5   &   $1\%$& $98\%$   \\ \hline
10   & $19\%$  & $99\%$    \\ \hline
15   & $26\%$ & $99\%$     \\ \hline
20  & $32\%$ & $99\%$   \\ \hline
\end{tabular}
\end{table}
%The FOM setting is 
{At the FOM level, we use} 
the EFR {strategy} presented in section \ref{sec:exampleFOM}. %\\ 
We recall the parameters used: The triangular mesh parameters are
 $h_{min} = 4.46 \cdot 10^{-3}$ and $h_{max} = 4.02 \cdot 10^{-2}$, %and by means of 
 {we use} a Taylor-Hood $\mathbb P^2 - \mathbb P^1$ %FE 
 {finite element} discretization, {and} we have $N_h \doteq N_h^{u} + N_h^p = 14053$ degrees of freedom. Moreover, %$\nu = 10^{-4}$ (
 $Re = 1000$, %$T=4 - \Delta t \sim 4$, 
 the time interval is $(0,4)$, 
 %for 
 $\Delta t = 4\cdot 10^{-4}$, {and} $\delta = C_{\delta} \delta^*$ with $C_{\delta} = \sqrt{11}$ and $\delta^*=4.46\cdot 10^{-3}$. The relaxation parameter is $\chi = 5\cdot \Delta t$. %\\
 
 For the EFR-EFR algorithm, we follow the consistency strategy proposed in \cite{Strazzullo20223148} and %these 
 {use the same} parameters %are used both at the FOM and 
 at the ROM level. 
 %Let us 
 {We} focus on the relative errors of %the 
 EFR-noEFR and EFR-EFR for velocity and pressure, %respectively 
 depicted in Figures \ref{fig:errror_efr_u} and \ref{fig:errror_efr_p}, {respectively}. The errors are computed for several values of {the number of} modes. For the sake of simplicity, we %have 
 {use} $r = r_u=r_s=r_p \in \{5, 10, 15, 20\}$ obtained by a POD approach over $1000$ equispaced snapshots in {the time interval} $(0,T)$. We choose some representative values for the {number of} basis functions %number and no energy criterion is followed. 
 {without employing a relative information criterion.}
 Indeed, from Table \ref{tab:A2energy}, we see that $r_u=20$ is not enough to preserve acceptable values of the %energy 
 {relative information} of the system. {Indeed, in} %In 
 order to represent %the 
 $98\%$ of the velocity %energy, an unbearable amount 
 {information, a large number}
 of basis functions is needed for the velocity, i.e., $r_u = 269$. For the pressure, %very 
 {a} few basis functions are enough to retain %the 
 $99\% $ of the %energy, however, the 
 {information.  The}
 results, {however,} are not satisfactory, as depicted in the relative errors plots in Figure \ref{fig:errror_efr_p}. 

 {The results in Figures  \ref{fig:errror_efr_u} and \ref{fig:errror_efr_p}
 show that EFR-EFR is more accurate than EFR-noEFR in approximating both the velocity and the pressure
 } 
 %Nevertheless, we observe a better representation of the EFR velocity if we employ EFR algorithm at the ROM level, too 
 (compare the cyan and orange lines or {the} teal and magenta %ones
 {lines}). %This complies with the conclusion of 
 {Thus, our numerical investigation yields the same conclusions and the investigation in} 
 \cite{Strazzullo20223148}: %EFR-EFR strategy is beneficial in terms of accuracy with respect to the EFR FOM simulation. 
 {EFR-EFR is more accurate than EFR-noEFR, i.e., using the same type of stabilization at the FOM and ROM levels yields more accurate results.}
 %Namely, numerical stabilization is helpful at the ROM level. 
 For example, focusing on the velocity profile, for $r = 10$, the EFR-EFR error is one order of magnitude lower than the %one of the 
 EFR-noEFR {error}. %strategy. 
 For $r = 15$, the gain is %of one order and an half. 
 {even larger.}
 This is true also for the pressure variable. %However, 
 {We note, however, that} the relative errors are large. Indeed, numerical oscillations can be observed at the ROM level, as depicted in Figure \ref{fig:EFRvsnoEFRrom}. It is clear that both approaches struggle to represent the EFR solution. 
 {The POD retained information and relative error plots suggest that this test problem represents a significant challenge for classical ROM strategies.}
 A different choice for the filter radius and the relaxation parameter at the reduced level %can 
 {could} improve the results. %Nevertheless, there is a need for a tailored reduction technique for this test case, as suggested from the POD retained energy and the related results in terms of relative errors. Anyway, this experimental analysis was beyond the goal of this section, where we only want to state the benefits of using the EFR strategy at the reduced level. 

\begin{figure}[H]
  \centering
  \includegraphics[width=0.49\textwidth]{img/uncontrolled/err10.pdf}
  \includegraphics[width=0.49\textwidth]{img/uncontrolled/err20.pdf}
  \caption{{Experiment A2. EFR-noEFR vs EFR. Velocity relative error for {the} EFR-noEFR and EFR %strategy 
  {strategies} with $C_{\delta} = \sqrt{11}$ %and 
  {for} $r \in \{5,10\}$ (left plot) and $r \in \{15,20\}$ (right plot).}}
  \label{fig:errror_efr_u}
  \end{figure} 

\begin{figure}[H]
  \centering
  \includegraphics[width=0.49\textwidth]{img/uncontrolled/err10p.pdf}
  \includegraphics[width=0.49\textwidth]{img/uncontrolled/err20p.pdf}
  \caption{{Experiment A2. EFR-noEFR vs EFR. Pressure relative error for {the} EFR-noEFR and EFR %strategy 
  {strategies} with $C_{\delta} = \sqrt{11}$ %and 
  {for} $r \in \{5,10\}$ (left plot) and $r \in \{15,20\}$ (right plot).}}
  \label{fig:errror_efr_p}
  \end{figure} 


